Tidal Signatures in the Faintest Milky Way Satellites: The Detailed Properties of Leo V, Pisces II and Canes Venatici II

We present deep wide-field photometry of three recently discovered faint Milky Way satellites: Leo V, Pisces II, and Canes Venatici II. Our main goals are to study the structure and star formation history of these dwarfs; we also search for signs of tidal disturbance. The three satellites have similar half-light radii ($\sim 60-90$ pc) but a wide range of ellipticities. Both Leo V and CVn II show hints of stream-like overdensities at large radii. An analysis of the satellite color-magnitude diagrams shows that all three objects are old ($>$ 10 Gyr) and metal-poor ([Fe/H] $\sim -2$), though neither the models nor the data have sufficient precision to assess when the satellites formed with respect to cosmic reionization. The lack of an observed younger stellar population ($\la 10$ Gyr) possibly sets them apart from the other satellites at Galactocentric distances $\ga 150$ kpc. We present a new compilation of structural data for all Milky Way satellite galaxies and use it to compare the properties of classical dwarfs to the ultra-faints. The ellipticity distribution of the two groups is consistent at the $\sim$2-$\sigma$ level. However, the faintest satellites tend to be more aligned toward the Galactic center, and those satellites with the highest ellipticity ($\ga 0.4$) have orientations ($\Delta \theta_{GC}$) in the range $20^{\circ} \lesssim \Delta \theta_{GC} \lesssim 40^{\circ}$. This latter observation is in rough agreement with predictions from simulations of dwarf galaxies that have lost a significant fraction of their dark matter halos and are being tidally stripped.

==> reply <==
Dr. de Grijs:
We are happy to resubmit our paper, 'Tidal Signatures in the Faintest Milky
Way Satellites: The Detailed Properties of Leo V, Pisces II and Canes
Venatici II', addressing all of the referee's comments.  

If necessary, the following is a written response to the referee
detailing what we have done.

Best regards,
David Sand


######

Dear Referee -- 

Thank you for your comments on 'Tidal Signatures in the Faintest Milky
Way Satellites: The Detailed Properties of Leo V, Pisces II and Canes
Venatici II'.  We have provided detailed replies to all of your
suggestions below -- indeed, I believe that all of your comments have
been incorporated into the text, at least to some degree.  Thank you.

>-- abstract, sentence 2: I find the last part of this sentence
>    somewhat misleading given the large uncertainty on Leo V's
>    ellipticity.  The real value and its uncertainty should be quoted
>    instead of the vague "~0.5" statement or, if the authors do not
>    want to choose between their two models, it should at least be
>    stated that their uncertainties are large, of the order of 0.2.

We have removed the offending clause which indicates Leo V has an
ellipticity of ~0.5.  We agree that its ellipticity is still
ambiguous.

>-- section 1, last paragraph: 
>* "A outline" -> "An outline"

Done, thanks.

>-- section 3: * Using known globular clusters (GCs) to comparatively
>determine the relative distance to the dwarf galaxies is a neat way to
>avoid unnecessary uncertainties but, once the distances are put on a
>global scale, the uncertainties on the globular clusters' distance
>moduli should be taken into account.  This is made particularly clear
>by the comment on literature values for the M92 distance modulus that
>differ by ~0.15.  So the distance uncertainties to the three dwarf
>galaxies are currently underestimated and should be updated to account
>for the GCs' distance moduli uncertainties.  From a quick look at the
>GC papers listed in section 3, it seems that these should be of the
>order of ~0.1 mag.  I would also like to point out that the value of
>the M92 distance modulus quoted from di Cecco et al. (2010) is an
>assumption of that paper and not the result of modeling.  Another
>source for this distance modulus (and a well-determined uncertainty
>for it) would be more relevant in the context of the Sand et
>al. paper.

This was fair and straightforward to implement.  First, the M92
distance modulus of di Cecco et al. (2010) was indeed an assumption,
but was similar to the $\mu=14.75$ mag found by Kraft & Ivans (2003).
We have adopted this reference and altered our values
accordingly.

Second, we have now included uncertainties in our assumed globular
cluster distances, and added these uncertainties in quadrature with
our final uncertainties on the distance to the three dwarfs studied in
our paper.  The text, and Table 5 have been updated accordingly.

>  * As a follow-up to this comment, it would be useful if Table 5 were
>    to also list the measured distance moduli and not just the
>    distances.

No problem.  Done.

>-- section 3, paragraph 3: * systematics should not be added in
>quadrature, but linearly, to the uncertainties.

We have now linearly added the systematic uncertainty associated with
the metallicity-luminosity relation of HB stars, rather than adding in
quadrature.

>-- section 4.1: * I wonder why the authors have decided to use a
>bootstrapping method to derive the uncertainties on the structural
>parameters when the maximum likelihood technique used to derive the
>parameters de facto gives the evolution of the likelihood in
>parameter space and, therefore, provides a direct means to measure
>the uncertainties without having to resort to a bootstrap method.

There are a couple of reasons why we do bootstrap resampling.  First,
it is quite time consuming to sample the likelihood around the maximum
when you are dealing with a multi-dimensional space -- as pointed out
by Munoz et al. 2010, who have also adopted a bootstrap technique
similar to our own.  

Second, Martin et al. 2008 have assumed that the structural parameters
behave like Gaussians near maximum, so that the log-likelihood behaves
like a chi-squared distribution.  It has been our experience, as we
discuss in Sand et al. 2009 (and see that paper's Figure 6), that this
might really underestimate the errors in their parameter estimation --
by a factor of 4-5 for Hercules, in that case.  Bootstrap resampling,
by its nature, will not suffer the same problem.

We believe that a systematic study comparing the bootstrap resampling
method of parameter estimation with the Martin et al. assumption of
Gaussianity would be important to do, especially if many more dwarfs
are forthcoming in the LSST era.  However, this is well beyond the
scope of the current work.


>  * In order to get a better grasp on the quality of the structural
>    parameter fits, I would like another Figure to be added, showing
>    the marginalized 2d likelihood contours for the structural
>    parameters &#x00E0; la Figure 13 of Martin, de Jong & Rix (2008;
>    at least for the position angle, the ellipticity and the half
>    light radius).  These would help the reader to judge the quality
>    of the fit in a way that Figure 2 alone cannot convey.

We have added this figure (the current Figure 3), although the contours are a little ratty.

>  * penultimate paragraph: Contrary to what is written in this
>    paragraph (and as far as I can tell from Figure 2) the data
>    presented in the paper do not follow the 3 requirements of Munoz
>    et al. (2012) to achieve ~10% precision on the structural
>    parameter determination.  From Figure 2, I estimate that the
>    central density contrast over the background is only ~10, and not
>    20.  This could explain why the structural parameters have
>    uncertainties larger than ~10%.

The referee is correct, and we have altered the text accordingly.

> * last paragraph: The fact the Okamoto et al. (2011) have binned and
>     smoothed their data could explain the difference in the measured
>     ellipticity of CVnII.  Martin, de Jong & Rix (2008; Figure 2)
>     have shown that the Maximum Likelihood technique used by Sand et
>     al. is far more reliable in the case of systems with a few
>     hundred stars.

Yes, we agree.  We have now mentioned this in the text, along with the
Martin et al. reference.

>-- section 4.2: * paragraph 2: "into 0.15 x 0.15 magnitude bins"
>should be "into 0.15 x 0.15 color-magnitude bins"

Done.

>  * penultimate paragraph: Since the matched filtered maps of Figure 3
>    have been smoothed, the values contained in different pixels are
>    now correlated, rendering the modes that are determined from the
>    maps meaningless.  Smoothing the data tends to boost the
>    significance of any deviation from a flat map especially if the
>    deviation has a size and shape close to these of the smoothing
>    kernel.  The authors haven't really relied on the significance of
>    the contours, which is a good thing, but I fear that keeping the
>    false denomination of 3, 4, 5,...-sigma contours could lead some
>    readers to assume that the stream-like overdensity in the maps
>    really are 3, 4, 5-sigma detections, which would be wrong.  I
>    suggest not smoothing the maps at all (they may look less pretty,
>    but the significance of the detections they contain will be much
>    more reliable), or dropping the "n-sigma contour" denomination
>    completely, maybe in favor of 10, 20,... % more signal that the
>    background?

We smoothed the data precisely for the same reason that the referee
mentioned -- 'Smoothing the data tends to boost the significance of
any deviation from a flat map especially if the deviation has a size
and shape close to these of the smoothing kernel' -- which we
considered a plus, in contrast to the referee.  We also disagree with
the statement made by the referee that this make the maps
'meaningless'.  We point out that the original matched-filter analysis
of Rockosi et al. 2002, on which our technique is based, also smoothed
their data of Palomar 5 to search for and understand the morphology of
its tidal tails.  We also point out our previous work (Sand et
al. 2009; 2010) where we have implemented simulations of 'fake
streams' and other structures to see how well we can recover extended
structure in our smoothed maps.

That said, we have no problem presenting un-smoothed maps, and so have
now put them in the paper -- along with our smoothed maps -- and
updated the text accordingly.

>-- section 4.2.1: * I am not entirely convinced by the comparison
>between the distribution of potential> Leo V BHB stars and that of
>its bulk population.  Do the authors account for the possibility that
>some of the stars in the BHB selection box could be contaminants?  My
>understanding is that they do not since the contamination/background
>level, \Sigma_b, fitted from the Leo V red giant branch and main
>sequence turn-off stars will be different from the BHB contamination
>level.  Although it is unlikely that many contaminants are present in
>the BHB selection box, I wonder what the effect of a single
>contaminant would be on the test performed by the authors and by how
>much the low probability they measure would be inflated.  May I
>suggest another possible test, namely to determine the structural
>parameters of the BHB-candidate-star distribution with the maximum
>likelihood algorithm that was used to determine the structure of
>dwarf galaxies and includes a background contamination term?  Given
>the small number of BHB-candidate stars, the measured half-light
>radius is likely to have large uncertainties, but that would still
>formally allow for a direct measure of the significance of any
>difference between the half-light radius of BHB-candidate stars and
>that measured for the bulk of Leo V stars.  This test could either
>replace or be added to the test current presented in this sub-section

We have taken the referee's suggestion and run our ML structural code
on the BHB stars directly.  Doing this, the extended nature of our Leo V BHB
stars diminishes to the ~1.8 sigma level.  We have amended the text
accordingly.  We have also dropped the clause in the abstract
suggesting that Leo~V had an extended BHB distribution.

>  * last paragraph: Independently of my comment above, I believe that
>    what the authors mean is that "...there is only a 0.4% (0.3%)
>    chance of getting a BHB sample with *an observed median radius
>    that is at least as small as that measured for the bulk of Leo V
>    stars...*"

We have made this change to the text.

>-- section 5.1: * paragraph 2: The "field" contamination that is
>removed from the Hess diagrams of Figure 4 is built from regions
>outside a radius of 8 arcminutes from the dwarf galaxies' centers
>whereas it was built from the regions outside a radius of 10
>arcminutes in the last paragraph of section 2.1.  Why the difference?

There is no reason for the difference, other than the fact that the
two Hess diagrams were constructed from different plotting codes.
They are now both made with background regions outside a radius of 8
arc min.  This results in only superficial changes to Figure 1.

>  * paragraphs 3 and onwards: I think this subsection could be
>    shortened as the authors quickly reach the limit of what can be
>    said star-formation-wise from main-sequence turnoff, ground-based
>    photometry of such faint systems.  In particular, I don't find the
>    paragraphs individually detailing the comments on the three dwarfs
>    particularly useful; they could be advantageously summarized and
>    merged with the penultimate paragraph of the sub-section which
>    presents the conclusion of the comparison with isochrones.

We do not have a problem with this suggestion.  We have removed the
paragraphs on individual objects and simply present a summary of our
results, since they do not vary significantly from object to object.

>-- section 5.2: * Even though it likely won't change the results, the
>distance modulus uncertainties should also be accounted for when
>determining the uncertainties on the absolute magnitudes of the
>dwarf.

We have now included distance modulus uncertainties into our absolute
magnitude measurements, although they do not formally change our
uncertainties at the single significant digit level at which we are
reporting our results.  The text of Section 5.2 has been updated.

>-- section 6.1: * This is the section of the discussion where I feel
>that the authors sometimes reach stronger conclusions than are
>warranted by their data set.  Admittedly the authors do make an effort
>to keep the discussion balanced, but I wonder what the goal of the
>discussion in paragraph 3 is when the authors have explained earlier
>that their star-formation analysis is only qualitative (sub-section
>5.1) and when paragraph 4 of section 6.1 correctly points out that a
>small but meaningful fraction of intermediate-age stars could have
>gone undetected, thereby undermining the conclusions of paragraph 3.
>Without a statistical analysis of the CMD of the dwarf galaxies
(&#x00E0; la, e.g., Dolphin 2002, de Jong et al. 2008), it seems that
>only speculations can be made about the impact of the environment on
>the star-formation history of these systems and whether they differ
>from brighter and better known MW dwarf galaxies.  

We are a little confused by the referee's concern here.  We do not
reach any strong conclusions, and we take a whole paragraph to explain
the limitations of our current SF analysis (and you yourself say our
discussion is balanced).  For this reason, we have left this section
largely alone (except for an occasional phrase to soften/reemphasize
the qualitative nature of our discussion).  As you will see below, we
have also softened other parts of the dicussion.  Since the referee
said we can take or leave this comment, we hope he/she is satisfied.

>Parts of paragraph
>5 are also more strongly worded than the data warrants: the
>metallicity of CVnII being 0.2 dex higher than the mean of the Kirby
>et al. (2011) relation is unlikely to be significant given the scatter
>in this relation (at least ~0.3 dex).  Even the difference of ~0.5 dex
>between the Walker et al. (2009a) Leo V metallicity measurement and
>the Kirby et al. (2011) relation may not be very significant once one
>accounts for the uncertainties on the measurement (0.2 dex) and likely
>systematics between the different models used to determine
>metallicities in these two papers.  I do not mean to tell the authors
>what they should put in their discussion and I will leave them to
>decide what they wish to keep in this sub-section, but I feel that the
>text would benefit from its strong conclusions being toned down to
>more directly reflect the results of the paper.

We agree with the referee that one should not over-interpret our
discussion about CVnII and Leo V being outliers in [Fe/H] vs. L space.
However, we do feel it is important to make connections, when
plausible, between our directly observed hints of stellar mass loss
with other indirect indications.  It is important to have balance here
and we have softened the paragraph by adding a sentence explicitly
stating that neither Leo V or CVn II are strong outliers from the
Kirby relation.  Hopefully the referee agrees that this is a step in
the right direction.

>-- section 6.2: * The significance of the difference between the mean
>ellipticities of the faint and bright MW satellites has been
>erroneously determined.  If the two means are mean1 and mean2, with
>associated uncertainties delta1 and delta2, the significance in
>"number of sigmas" should then be (under the usual assumption of
>Gaussianity): significance = |mean1-mean2| / sqrt(delta1^2 + delta2^2)

>This means that the two means are different at the 2.1-sigma level
>  (and not the 1.8-sigma level).  The same applies to the study of the
>  spreads, leading to a difference at the 1.6-sigma level between the
>  determined scatters (and not at the 1.4-sigma level).  I'm not sure
>  that this indicates "no significant difference" between the two
>  populations, but that it is in fact in the blurry region where
>  things can be argued one way or another.

The referee is correct (I must have made a dumb mistake).  Thanks.
The text has been adjusted accordingly.
